Spatial Reasoner: A 3D Inference Pipeline for XR Applications

Modern extended reality XR systems provide rich analysis of image data and fusion of sensor input and demand AR/VR applications that can reason about 3D scenes in a semantic manner. We present a spatial reasoning framework that bridges geometric facts with symbolic predicates and relations to handle key tasks such as determining how 3D objects are arranged among each other ('on', 'behind', 'near', etc.). Its foundation relies on oriented 3D bounding box representations, enhanced by a comprehensive set of spatial predicates, ranging from topology and connectivity to directionality and orientation, expressed in a formalism related to natural language. The derived predicates form a spatial knowledge graph and, in combination with a pipeline-based inference model, enable spatial queries and dynamic rule evaluation. Implementations for client- and server-side processing demonstrate the framework's capability to efficiently translate geometric data into actionable knowledge, ensuring scalable and technology-independent spatial reasoning in complex 3D environments. The Spatial Reasoner framework is fostering the creation of spatial ontologies, and seamlessly integrates with and therefore enriches machine learning, natural language processing, and rule systems in XR applications.

==> Apendix_saved.tex <==
\section{Appendix}

This appendix compiles the key spatial predicates used throughout our framework. Each subsection presents a category of predicates with a table summarizing (i) the predicate name, (ii) the spatial relation it encodes, (iii) a concise specification, and (iv) an illustrative visual.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 3) Adjacency Table
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
\centering 
\caption{Adjacency Predicates}
\label{tab:adjacency}
\begin{tabular}{M{1.4cm} L{1.2cm} L{2.cm} M{2.2cm}}
\toprule
\textbf{Predicate} & \textbf{Relation} & \textbf{Specification} & \textbf{Visual} \\
\midrule
\texttt{leftside} 
& subj is at \textbf{leftside} of obj 
& \begin{tblitemize}
        \item center is in .l sector
        \item is near, not overlapping
        \item valid in OCS
    \end{tblitemize}
& \includegraphics[width=2.3cm]{images/leftside.png} \\
%
\texttt{rightside} 
& subj is at \textbf{rightside} of obj 
& \begin{tblitemize}
    \item center is in .r sector
    \item is near, not overlapping
    \item valid in OCS
\end{tblitemize} 
& \includegraphics[width=2.3cm]{images/rightside.png} \\
%
\texttt{frontside} 
& subj is at \textbf{frontside} of obj 
& \begin{tblitemize}
    \item center in .a sector
    \item near, not overlapping
    \item valid in OCS
\end{tblitemize} 
& \includegraphics[width=2.3cm]{images/frontside.png} \\
%
\texttt{backside} 
& subj is at \textbf{backside} of obj 
& \begin{tblitemize}
    \item center in .b sector
    \item near, not overlapping
    \item valid in OCS
\end{tblitemize} 
& \includegraphics[width=2.3cm]{images/backside.png} \\
%
\texttt{beside} 
& subj is \textbf{beside} obj 
& \begin{tblitemize}
    \item near, not above/below
    \item not overlapping
    \item valid in WCS/OCS/ECS
\end{tblitemize} 
& \includegraphics[width=2.3cm]{images/beside.png} \\
%
\texttt{upperside} 
& subj is at \textbf{upperside} of obj 
& \begin{tblitemize}
    \item center in .o sector
    \item near, not overlapping
    \item valid in WCS/OCS/ECS
\end{tblitemize} 
& \includegraphics[width=2.0cm]{images/upperside.png} \\
%
\texttt{lowerside} 
& subj is at \textbf{lowerside} of obj 
& \begin{tblitemize}
    \item center in .u sector
    \item near, not overlapping
    \item valid in WCS/OCS/ECS
\end{tblitemize} 
& \includegraphics[width=2.0cm]{images/lowerside.png} \\
%
\texttt{ontop} 
& subj is \textbf{ontop} of obj 
& \begin{tblitemize}
    \item center in .o sector
    \item near, not overlapping
    \item min dist $<$ max gap
\end{tblitemize} 
& \includegraphics[width=2.0cm]{images/ontop.png} \\
%
\texttt{beneath} 
& subj is \textbf{beneath} obj 
& \begin{tblitemize}
    \item center in .u sector
    \item near, not overlapping
    \item min dist $<$ max gap
\end{tblitemize} 
& \includegraphics[width=2.0cm]{images/beneath.png} \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Adjacency Predicates}
Adjacency predicates concern objects that are close but not overlapping, with specification for leftside, rightside, etc.

\subsection{Assembly Predicates}
Assembly predicates describe overlap, containment, and adjacency in terms of bounding-box relationships.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 5) Assembly Table
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering       
\caption{Assembly Predicates}
\label{tab:assembly}
\begin{tabular}{M{1.6cm} L{1.5cm} L{2.0cm} M{2.2cm}}
\toprule
\textbf{Predicate} & \textbf{Relation} & \textbf{Specification} & \textbf{Visual} \\
\midrule
\texttt{disjoint}
& subj is \textbf{disjoint} from obj
& \begin{tblitemize}
    \item no overlap
    \item valid in WCS, OCS, ECS
\end{tblitemize}
& \includegraphics[width=2.2cm]{images/ahead.png} \\
%
\texttt{inside}
& subj is \textbf{inside} obj
& \begin{tblitemize}
    \item bounding box inside
    \item valid in WCS, OCS, ECS
\end{tblitemize}
& \includegraphics[width=2.2cm]{images/inside.png} \\
%
\texttt{containing}
& subj is \textbf{containing} obj
& \begin{tblitemize}
    \item is containing
    \item valid in WCS, OCS, ECS
\end{tblitemize}
& \includegraphics[width=2.2cm]{images/containing.png} \\
%
\texttt{overlapping}
& subj is \textbf{overlapping} with obj
& \begin{tblitemize}
    \item partial overlap
    \item not crossing fully
\end{tblitemize}
& \includegraphics[width=2.2cm]{images/left.png} \\
%
\texttt{crossing}
& subj is \textbf{crossing} obj
& \begin{tblitemize}
    \item is crossing
    \item valid in WCS, OCS, ECS
\end{tblitemize}
& \includegraphics[width=2.2cm]{images/crossing.png} \\
%
\texttt{touching}
& subj is \textbf{touching} obj
& \begin{tblitemize}
    \item edge/corner contact
    \item min distance $<$ max gap
\end{tblitemize}
& \includegraphics[width=2.2cm]{images/touching.png} \\
%
\texttt{meeting}
& subj is \textbf{meeting} obj
& \begin{tblitemize}
    \item face contact
    \item angle diff $<$ max angle
\end{tblitemize}
& \includegraphics[width=2.2cm]{images/meeting.png} \\
\bottomrule
\end{tabular}%
\end{table}


\subsection{Directionality Predicates}
Directionality predicates indicate left/right or front/back type relationships. They can also define above/over and below/under in world or local object coordinates.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 2) Directionality Table
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering      
\caption{Directionality Predicates}
\label{tab:directionality}
\begin{tabular}{M{1.0cm} L{1.2cm} L{2.6cm} M{2.3cm}}
\toprule
\textbf{Predicate} & \textbf{Relation} & \textbf{Specification} & \textbf{Visual} \\
\midrule
\texttt{left}
& subj is \textbf{left} of obj
& \begin{tblitemize}
    \item center of subject is left
    \item may overlap, no distance condition
    \item valid in OCS
\end{tblitemize}
& \includegraphics[width=2.3cm]{images/left.png} \\
%
\texttt{right}
& subj is \textbf{right} of obj
& \begin{tblitemize}
    \item center of subject is right
    \item may overlap, no distance condition
    \item valid in OCS
\end{tblitemize}
& \includegraphics[width=2.1cm]{images/right.png} \\
%
\texttt{ahead}
& subj is \textbf{ahead} of obj
& \begin{tblitemize}
    \item center of subject is ahead
    \item may overlap, no distance condition
    \item valid in OCS
\end{tblitemize}
& \includegraphics[width=2.1cm]{images/ahead.png} \\
%
\texttt{behind}
& subj is \textbf{behind} obj
& \begin{tblitemize}
    \item center of subject is behind
    \item may overlap, no distance condition
    \item valid in OCS
\end{tblitemize}
& \includegraphics[width=2.1cm]{images/behind.png} \\
%
\texttt{above}/ \texttt{over}
& subj is \textbf{above/ over} obj
& \begin{tblitemize}
    \item center is above object
    \item no distance condition
    \item valid in WCS/OCS/ECS
\end{tblitemize}
& \includegraphics[width=1.8cm]{images/above.png} \\
%
\texttt{below}/ \texttt{under}
& subj is \textbf{below/ under} obj
& \begin{tblitemize}
    \item center is below object
    \item no distance condition
    \item valid in WCS/OCS/ECS
\end{tblitemize}
& \includegraphics[width=1.8cm]{images/below.png} \\
\bottomrule
\end{tabular}
\end{table}


\subsection{Connectivity Predicates}
Connectivity predicates describe direct contacts like being “on” or “in,” considering minimal gaps and bounding-box containment.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 6) Connectivity Table
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
\centering       
\caption{Connectivity Predicates}
\label{tab:connectivity}
\begin{tabular}{M{1.0cm} L{1.0cm} L{2.5cm} M{2.2cm}}
\toprule
\textbf{Predicate} & \textbf{Relation} & \textbf{Specification} & \textbf{Visual} \\
\midrule
\texttt{on}
& subj is \textbf{on} obj
& \begin{tblitemize}
    \item is on top
    \item near, min distance $<$ max gap
    \item valid in WCS/OCS/ECS
\end{tblitemize}
& \includegraphics[width=2.2cm]{images/on.png} \\
%
\texttt{at}
& subj is \textbf{at} obj
& \begin{tblitemize}
    \item is beside
    \item is meeting
    \item min distance $<$ max gap
\end{tblitemize}
& \includegraphics[width=2.2cm]{images/at.png} \\
%
\texttt{by}
& subj is \textbf{by} obj
& \begin{tblitemize}
    \item is touching
    \item min distance $<$ max gap
\end{tblitemize}
& \includegraphics[width=2.2cm]{images/by.png} \\
%
\texttt{in}
& subj is \textbf{in} obj
& \begin{tblitemize}
    \item bounding box inside
    \item valid in WCS/OCS/ECS
\end{tblitemize}
& \includegraphics[width=2.2cm]{images/in.png} \\
\bottomrule
\end{tabular}%
\end{table}

\subsection{Visibility Predicates}
Visibility predicates focus on how an object is perceived from a specific viewpoint or “ego” coordinate system.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 7) Visibility Table
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
\centering     
\caption{Visibility Predicates}
\label{tab:visibility}
\begin{tabular}{M{1.3cm} L{1.4cm} L{2.0cm} M{2.2cm}}
\toprule
\textbf{Predicate} & \textbf{Relation} & \textbf{Specification} & \textbf{Visual} \\
\midrule
\texttt{infront}
& subj is \textbf{in front} of obj
& \begin{tblitemize}
    \item seen in front
    \item valid in ECS
\end{tblitemize}
& \includegraphics[width=2.2cm]{images/infront.png} \\
%
\texttt{atrear}
& subj is \textbf{at rear} of obj
& \begin{tblitemize}
    \item seen behind
    \item valid in ECS
\end{tblitemize}
& \includegraphics[width=2.2cm]{images/atrear.png} \\
%
\texttt{seenright}
& subj is \textbf{seen right} of obj
& \begin{tblitemize}
    \item angle from observer
    \item valid in ECS
\end{tblitemize}
& \includegraphics[width=2.0cm]{images/seenright.png} \\
%
\texttt{seenleft}
& subj is \textbf{seen left} of obj
& \begin{tblitemize}
    \item angle from observer
    \item valid in ECS
\end{tblitemize}
& \includegraphics[width=2.2cm]{images/seenleft.png} \\
\bottomrule
\end{tabular}%
\end{table}

\subsection{Sectoriality Predicates}
Sectoriality predicates split the space around an object into finer “3D sectors” (e.g., bru standing for behind-right-under) for more granular positional reasoning.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 8) Sectoriality Table
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
\centering         
\caption{Sectoriality Predicates}
\label{tab:sectoriality}
\begin{tabular}{M{0.8cm} L{1.5cm} L{2cm} M{2.2cm}}
\toprule
\textbf{Predicate} & \textbf{Relation} & \textbf{Specification} & \textbf{Visual} \\
\midrule
\texttt{o}
& subj in sector \textbf{o} of obj
& \begin{tblitemize}
    \item center in .o
    \item is over
    \item valid in OCS
\end{tblitemize}
& \includegraphics[width=2.2cm]{images/in_o.png} \\
%
\texttt{br}
& subj in sector \textbf{br} of obj
& \begin{tblitemize}
    \item center in .br
    \item behind right
    \item valid in OCS
\end{tblitemize}
& \includegraphics[width=2.2cm]{images/in_br.png} \\
%
\texttt{bru}
& subj in sector \textbf{bru} of obj
& \begin{tblitemize}
    \item center in .bru
    \item behind right under
    \item valid in OCS
\end{tblitemize}
& \includegraphics[width=2.2cm]{images/in_bru.png} \\
\bottomrule
\end{tabular}%
\end{table}

\subsection{Proximity Predicates}
Proximity predicates capture whether two objects are near or far from each other, typically comparing center distances against a predefined threshold.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 1) Proximity Table
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
\centering
\caption{Proximity Predicates}
\label{tab:proximity}
\begin{tabular}{M{1.0cm} L{1.1cm} L{2cm} M{3.0cm}}
\toprule
\textbf{Predicate} & \textbf{Relation} & \textbf{Specification} & \textbf{Visual} \\
\midrule
\texttt{near} 
& subj is \textbf{near} obj
& \begin{tblitemize}
    \item center distance $<$ nearby condition
    \item not in \texttt{.i} sector
    \item \texttt{delta} = center distance
\end{tblitemize}
& \includegraphics[width=3.0cm]{images/near.png} \\
%
\texttt{far} 
& subj is \textbf{far} from obj
& \begin{tblitemize}
    \item center distance $>$ nearby condition
    \item not near
    \item \texttt{delta} = center distance
\end{tblitemize}
& \includegraphics[width=3.0cm]{images/far.png} \\
\bottomrule
\end{tabular}%
\end{table}



\subsection{Comparability Predicates}
Comparability predicates compare two objects with respect to size, length, volume, and so on.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 9) Comparability Table
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
\centering
\renewcommand{\arraystretch}{1.5}
\caption{Comparability Predicates (Compact Version)}
\label{tab:comparability}
\begin{tabular}{M{1.4cm} L{2.0cm} P{3.6cm}}
\toprule
\textbf{Predicate} & \textbf{Relation} & \textbf{Specification} \\
\midrule
\texttt{shorter}
  & subj is \textbf{shorter} than obj
  & length is shorter; \texttt{delta} = height difference \\[2pt]
\texttt{longer}
  & subj is \textbf{longer} than obj
  & length is larger; \texttt{delta} = length difference \\[2pt]
\texttt{taller}
  & subj is \textbf{taller} than obj
  & height is larger; \texttt{delta} = height difference \\[2pt]
\texttt{thinner}
  & subj is \textbf{thinner} than obj
  & footprint is smaller; \texttt{delta} = footprint difference \\[2pt]
\texttt{wider}
  & subj is \textbf{wider} than obj
  & footprint is larger; \texttt{delta} = footprint difference \\[2pt]
\texttt{smaller}
  & subj is \textbf{smaller} than obj
  & volume is smaller; \texttt{delta} = volume difference \\[2pt]
\texttt{bigger}
  & subj is \textbf{bigger} than obj
  & volume is bigger; \texttt{delta} = volume difference \\[2pt]
\texttt{fitting}
  & subj is \textbf{fitting} into obj
  & is fitting within; \texttt{delta} = volume difference \\[2pt]
\texttt{exceeding}
  & subj is \textbf{exceeding} obj
  & not fitting within; \texttt{delta} = volume difference \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Similarity Predicates}
Similarity predicates check whether objects share dimensions, positions, or surface properties within a chosen tolerance.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 10) Similarity Table
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
\centering
\renewcommand{\arraystretch}{1.5}
\caption{Similarity Predicates (Compact Version)}
\label{tab:similarity}
\begin{tabular}{M{1.9cm} L{1.9cm} P{3.6cm}}
\toprule
\textbf{Predicate} & \textbf{Relation} & \textbf{Specification} \\
\midrule
\texttt{sameheight}   & subj has \textbf{sameheight} as obj   & height difference $<\!$ max gap \\[2pt]
\texttt{samewidth}    & subj has \textbf{samewidth} as obj    & width difference $<\!$ max gap \\[2pt]
\texttt{samedepth}    & subj has \textbf{samedepth} as obj    & depth difference $<\!$ max gap \\[2pt]
\texttt{samelength}   & subj has \textbf{samelength} as obj   & length difference $<\!$ max gap \\[2pt]
\texttt{sameperimeter}& subj has \textbf{sameperimeter} as obj& perimeter diff $< 4\times$(max gap) \\[2pt]
\texttt{samefront}    & subj has \textbf{samefront} as obj    & front area diff $<\!$ (max gap)$^2$ \\[2pt]
\texttt{sameside}     & subj has \textbf{sameside} as obj     & side area diff $<\!$ (max gap)$^2$ \\[2pt]
\texttt{samefootprint}& subj has \textbf{samefootprint} as obj& base area diff $<\!$ (max gap)$^2$ \\[2pt]
\texttt{samesurface}  & subj has \textbf{samesurface} as obj  & surface diff $< 3\times$(max gap)$^2$ \\[2pt]
\texttt{samevolume}   & subj has \textbf{samevolume} as obj   & volume diff $<\!$ (max gap)$^3$ \\[2pt]
\texttt{samecuboid}   & subj has \textbf{samecuboid} as obj   & same width, height, and depth \\[2pt]
\texttt{congruent}    & subj is \textbf{congruent} with obj   & same dimensions + orientation \\[2pt]
\texttt{sameposition} & subj has \textbf{sameposition} as obj & position diff $<\!$ max gap \\[2pt]
\texttt{samecenter}   & subj has \textbf{samecenter} as obj   & center diff $<\!$ max gap \\[2pt]
\texttt{sameshape}    & subj has \textbf{sameshape} as obj    & same shape label \\
\bottomrule
\end{tabular}
\end{table}

\begin{table*}[htbp]
\centering
\renewcommand{\arraystretch}{2.0}
\caption{Available operations in inference pipeline of Spatial Reasoner}
\label{tab:inference-ops}
\begin{tabular}{p{1.3cm} p{7.3cm} p{7.5cm}}
\hline
\textbf{Op} & \textbf{Syntax} & \textbf{Examples} \\
\hline
\texttt{adjust} & \texttt{adjust(\textit{settings})} & \texttt{adjust(max gap 0.05)} \newline \texttt{adjust(sector fixed 1.2)} \newline \texttt{adjust(nearby dimension 2.0)} \newline \texttt{adjust(long ratio 4.0)} \newline\texttt{adjust(nearby limit 4.0; max gap 0.1)}\\
\texttt{deduce} & \texttt{deduce(\textit{relation-categories})} & \texttt{deduce(topology)} \newline \texttt{deduce(visibility comparability)} \newline \texttt{deduce(topology visibility similarity)} \\
\texttt{filter} & \texttt{filter(\textit{attribute-conditions})} & \texttt{filter(id == 'wall2')} \newline \texttt{filter(width > 0.5 AND height < 2.4)} \newline \texttt{filter(type == 'chair')} \newline \texttt{filter(thin AND volume > 0.4)} \\
\texttt{isa} & \texttt{isa(\textit{class-type})} & \texttt{isa('Bed')} \newline \texttt{isa(Furniture)} \newline \texttt{isa(Computer OR Monitor)} \\
\texttt{pick} & \texttt{pick(\textit{relation-conditions})} & \texttt{pick(near)} \newline \texttt{pick(ahead AND smaller)} \newline \texttt{pick(near AND (left OR right))}\\
\texttt{select} & \texttt{select(\textit{relations [? attribute-conditions]})} & \texttt{select(opposite)} \newline \texttt{select(ontop ? label == 'table')} \newline  \texttt{select(on ? type == 'floor')} \newline \texttt{select(ahead AND smaller ? footprint < 0.5)} \\
\texttt{sort} & \texttt{sort(\textit{object-attribute [comparator]})} & \texttt{sort(width)} \newline \texttt{sort(volume <)} \newline \texttt{sort(volume >)} \\
\texttt{sort} & \texttt{sort(\textit{relation-attribute [comparator steps]})} & \texttt{sort(near.delta)} \newline \texttt{sort(frontside.angle <)} \newline \texttt{sort(disjoint.delta > 2)} \\
\texttt{slice} & \texttt{slice(\textit{range})} & \texttt{slice(1)} \newline \texttt{slice(2..3)} \newline \texttt{slice(-1)} \\
\texttt{calc} & \texttt{calc(\textit{variable-assignments})} & \texttt{calc(cnt = count(objects))} \newline \texttt{calc(maxvol = max(objects.volume))} \\
\texttt{map} & \texttt{map(\textit{attribute-assignments})} & \texttt{map(shape = 'cylindrical')} \newline \texttt{map(type = 'bed'; shape = 'cubical')} \newline \texttt{map(weight = volume * 140.0)} \\
\texttt{produce} & \texttt{produce(\textit{relation : attribute-assignments})} & \texttt{produce(copy : id = 'copy'; y = 2.0)} \newline \texttt{produce(group : type = 'room')} \newline \texttt{produce(on : label = 'zone')} \newline \texttt{produce(by : label = 'corner'; h = 0.02)} \\
\texttt{reload} & \texttt{reload()} & \texttt{reload()} \\
\texttt{halt} & \texttt{halt()} & \texttt{halt()} \\
\texttt{log} & \texttt{log(3D base \textit{relations})} & \texttt{log(3D)} \newline \texttt{log(base)} \newline \texttt{log(3D near right)} \\
\hline
\end{tabular}
\end{table*}

\clearpage


==> tables.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 1) Proximity Table
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[htbp]
\centering
\footnotesize          % Make font smaller
\renewcommand{\arraystretch}{0.5} 
\caption{Proximity Predicates}
\label{tab:proximity}
\begin{tabular}{M{1.8cm} M{2.0cm} M{4cm} M{2.0cm}}
\toprule
\textbf{Predicate} & \textbf{Relation} & \textbf{Specification} & \textbf{Visual} \\
\midrule
\texttt{near} 
& subj is \textbf{near} obj
& \begin{itemize}
    \item center distance $<$ nearby condition
    \item not in \texttt{.i} sector
    \item \texttt{delta} = center distance
\end{itemize}
& \includegraphics[width=2.0cm]{images/near.png} \\
%
\texttt{far} 
& subj is \textbf{far} from obj
& \begin{itemize}
    \item center distance $>$ nearby condition
    \item not near
    \item \texttt{delta} = center distance
\end{itemize}
& \includegraphics[width=2.0cm]{images/far.png} \\
\bottomrule
\end{tabular}%

\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 2) Directionality Table
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[htbp]
\centering
\footnotesize          % Make font smaller
\renewcommand{\arraystretch}{0.5} 
\caption{Directionality Predicates}
\label{tab:directionality}
\begin{tabular}{M{1.8cm} M{2.0cm} M{4cm} M{2.0cm}}
\toprule
\textbf{Predicate} & \textbf{Relation} & \textbf{Specification} & \textbf{Visual} \\
\midrule
\texttt{left}
& subj is \textbf{left} of obj
& \begin{itemize}
    \item center of subject is left
    \item may overlap, no distance condition
    \item valid in OCS
\end{itemize}
& \includegraphics[width=2.0cm]{images/left.png} \\
%
\texttt{right}
& subj is \textbf{right} of obj
& \begin{itemize}
    \item center of subject is right
    \item may overlap, no distance condition
    \item valid in OCS
\end{itemize}
& \includegraphics[width=2.0cm]{images/right.png} \\
%
\texttt{ahead}
& subj is \textbf{ahead} of obj
& \begin{itemize}
    \item center of subject is ahead
    \item may overlap, no distance condition
    \item valid in OCS
\end{itemize}
& \includegraphics[width=2.0cm]{images/ahead.png} \\
%
\texttt{behind}
& subj is \textbf{behind} obj
& \begin{itemize}
    \item center of subject is behind
    \item may overlap, no distance condition
    \item valid in OCS
\end{itemize}
& \includegraphics[width=2.0cm]{images/behind.png} \\
%
\texttt{above}/\texttt{over}
& subj is \textbf{above/over} obj
& \begin{itemize}
    \item center is above object
    \item no distance condition
    \item valid in WCS/OCS/ECS
\end{itemize}
& \includegraphics[width=2.0cm]{images/above.png} \\
%
\texttt{below}/\texttt{under}
& subj is \textbf{below/under} obj
& \begin{itemize}
    \item center is below object
    \item no distance condition
    \item valid in WCS/OCS/ECS
\end{itemize}
& \includegraphics[width=2.0cm]{images/below.png} \\
\bottomrule
\end{tabular}%

\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 3) Adjacency Table
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[htbp]
\centering
\footnotesize          % Make font smaller
\renewcommand{\arraystretch}{0.5} 
\caption{Adjacency Predicates}
\label{tab:adjacency}
\begin{tabular}{M{1.8cm} M{2.0cm} M{4cm} M{2.0cm}}
\toprule
\textbf{Predicate} & \textbf{Relation} & \textbf{Specification} & \textbf{Visual} \\
\midrule
\texttt{leftside} 
& subj is at \textbf{leftside} of obj 
& \begin{itemize}
    \item center is in .l sector
    \item is near, not overlapping
    \item valid in OCS
\end{itemize} 
& \includegraphics[width=2.0cm]{images/leftside.png} \\
%
\texttt{rightside} 
& subj is at \textbf{rightside} of obj 
& \begin{itemize}
    \item center is in .r sector
    \item is near, not overlapping
    \item valid in OCS
\end{itemize} 
& \includegraphics[width=2.0cm]{images/rightside.png} \\
%
\texttt{frontside} 
& subj is at \textbf{frontside} of obj 
& \begin{itemize}
    \item center in .a sector
    \item near, not overlapping
    \item valid in OCS
\end{itemize} 
& \includegraphics[width=2.0cm]{images/frontside.png} \\
%
\texttt{backside} 
& subj is at \textbf{backside} of obj 
& \begin{itemize}
    \item center in .b sector
    \item near, not overlapping
    \item valid in OCS
\end{itemize} 
& \includegraphics[width=2.0cm]{images/backside.png} \\
%
\texttt{beside} 
& subj is \textbf{beside} obj 
& \begin{itemize}
    \item near, not above/below
    \item not overlapping
    \item valid in WCS/OCS/ECS
\end{itemize} 
& \includegraphics[width=2.0cm]{images/beside.png} \\
%
\texttt{upperside} 
& subj is at \textbf{upperside} of obj 
& \begin{itemize}
    \item center in .o sector
    \item near, not overlapping
    \item valid in WCS/OCS/ECS
\end{itemize} 
& \includegraphics[width=2.0cm]{images/upperside.png} \\
%
\texttt{lowerside} 
& subj is at \textbf{lowerside} of obj 
& \begin{itemize}
    \item center in .u sector
    \item near, not overlapping
    \item valid in WCS/OCS/ECS
\end{itemize} 
& \includegraphics[width=2.0cm]{images/lowerside.png} \\
%
\texttt{ontop} 
& subj is \textbf{ontop} of obj 
& \begin{itemize}
    \item center in .o sector
    \item near, not overlapping
    \item min dist $<$ max gap
\end{itemize} 
& \includegraphics[width=2.0cm]{images/ontop.png} \\
%
\texttt{beneath} 
& subj is \textbf{beneath} obj 
& \begin{itemize}
    \item center in .u sector
    \item near, not overlapping
    \item min dist $<$ max gap
\end{itemize} 
& \includegraphics[width=2.0cm]{images/beneath.png} \\
\bottomrule
\end{tabular}%

\end{table*}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 5) Assembly Table
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[htbp]
\centering
\footnotesize          % Make font smaller
\renewcommand{\arraystretch}{0.5} 
\caption{Assembly Predicates}
\label{tab:assembly}
\begin{tabular}{M{1.8cm} M{2.0cm} M{4cm} M{2.0cm}}
\toprule
\textbf{Predicate} & \textbf{Relation} & \textbf{Specification} & \textbf{Visual} \\
\midrule
\texttt{disjoint}
& subj is \textbf{disjoint} from obj
& \begin{itemize}
    \item no overlap
    \item valid in WCS, OCS, ECS
\end{itemize}
& \includegraphics[width=2.0cm]{images/ahead.png} \\
%
\texttt{inside}
& subj is \textbf{inside} obj
& \begin{itemize}
    \item bounding box inside
    \item valid in WCS, OCS, ECS
\end{itemize}
& \includegraphics[width=2.0cm]{images/inside.png} \\
%
\texttt{containing}
& subj is \textbf{containing} obj
& \begin{itemize}
    \item is containing
    \item valid in WCS, OCS, ECS
\end{itemize}
& \includegraphics[width=2.0cm]{images/containing.png} \\
%
\texttt{overlapping}
& subj is \textbf{overlapping} with obj
& \begin{itemize}
    \item partial overlap
    \item not crossing fully
\end{itemize}
& \includegraphics[width=2.0cm]{images/left.png} \\
%
\texttt{crossing}
& subj is \textbf{crossing} obj
& \begin{itemize}
    \item is crossing
    \item valid in WCS, OCS, ECS
\end{itemize}
& \includegraphics[width=2.0cm]{images/crossing.png} \\
%
\texttt{touching}
& subj is \textbf{touching} obj
& \begin{itemize}
    \item edge/corner contact
    \item min distance $<$ max gap
\end{itemize}
& \includegraphics[width=2.0cm]{images/touching.png} \\
%
\texttt{meeting}
& subj is \textbf{meeting} obj
& \begin{itemize}
    \item face contact
    \item angle diff $<$ max angle
\end{itemize}
& \includegraphics[width=2.0cm]{images/meeting.png} \\
\bottomrule
\end{tabular}%

\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 6) Connectivity Table
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[htbp]
\centering
\footnotesize          % Make font smaller
\renewcommand{\arraystretch}{0.5} 
\caption{Connectivity Predicates}
\label{tab:connectivity}
\begin{tabular}{M{1.8cm} M{2.0cm} M{4cm} M{2.0cm}}
\toprule
\textbf{Predicate} & \textbf{Relation} & \textbf{Specification} & \textbf{Visual} \\
\midrule
\texttt{on}
& subj is \textbf{on} obj
& \begin{itemize}
    \item is on top
    \item near, min distance $<$ max gap
    \item valid in WCS/OCS/ECS
\end{itemize}
& \includegraphics[width=2.0cm]{images/on.png} \\
%
\texttt{at}
& subj is \textbf{at} obj
& \begin{itemize}
    \item is beside
    \item is meeting
    \item min distance $<$ max gap
\end{itemize}
& \includegraphics[width=2.0cm]{images/at.png} \\
%
\texttt{by}
& subj is \textbf{by} obj
& \begin{itemize}
    \item is touching
    \item min distance $<$ max gap
\end{itemize}
& \includegraphics[width=2.0cm]{images/by.png} \\
%
\texttt{in}
& subj is \textbf{in} obj
& \begin{itemize}
    \item bounding box inside
    \item valid in WCS/OCS/ECS
\end{itemize}
& \includegraphics[width=2.0cm]{images/in.png} \\
\bottomrule
\end{tabular}%

\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 7) Visibility Table
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[htbp]
\centering
\footnotesize          % Make font smaller
\renewcommand{\arraystretch}{0.5} 
\caption{Visibility Predicates}
\label{tab:visibility}
\begin{tabular}{M{1.8cm} M{2.0cm} M{4cm} M{2.0cm}}
\toprule
\textbf{Predicate} & \textbf{Relation} & \textbf{Specification} & \textbf{Visual} \\
\midrule
\texttt{infront}
& subj is \textbf{in front} of obj
& \begin{itemize}
    \item seen in front
    \item valid in ECS
\end{itemize}
& \includegraphics[width=2.0cm]{images/infront.png} \\
%
\texttt{atrear}
& subj is \textbf{at rear} of obj
& \begin{itemize}
    \item seen behind
    \item valid in ECS
\end{itemize}
& \includegraphics[width=2.0cm]{images/atrear.png} \\
%
\texttt{seenright}
& subj is \textbf{seen right} of obj
& \begin{itemize}
    \item angle from observer
    \item valid in ECS
\end{itemize}
& \includegraphics[width=2.0cm]{images/seenright.png} \\
%
\texttt{seenleft}
& subj is \textbf{seen left} of obj
& \begin{itemize}
    \item angle from observer
    \item valid in ECS
\end{itemize}
& \includegraphics[width=2.0cm]{images/seenleft.png} \\
\bottomrule
\end{tabular}%
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 8) Sectoriality Table
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[htbp]
\centering
\footnotesize          % Make font smaller
\renewcommand{\arraystretch}{0.5} 
\caption{Sectoriality Predicates}
\label{tab:sectoriality}
\begin{tabular}{M{1.8cm} M{2.0cm} M{4cm} M{2.0cm}}
\toprule
\textbf{Predicate} & \textbf{Relation} & \textbf{Specification} & \textbf{Visual} \\
\midrule
\texttt{o}
& subj in sector \textbf{o} of obj
& \begin{itemize}
    \item center in .o
    \item is over
    \item valid in OCS
\end{itemize}
& \includegraphics[width=2.0cm]{images/in_o.png} \\
%
\texttt{br}
& subj in sector \textbf{br} of obj
& \begin{itemize}
    \item center in .br
    \item behind right
    \item valid in OCS
\end{itemize}
& \includegraphics[width=2.0cm]{images/in_br.png} \\
%
\texttt{bru}
& subj in sector \textbf{bru} of obj
& \begin{itemize}
    \item center in .bru
    \item behind right under
    \item valid in OCS
\end{itemize}
& \includegraphics[width=2.0cm]{images/in_bru.png} \\
\bottomrule
\end{tabular}%
\end{table*}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 9) Comparability Table
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[htbp]
\centering
\footnotesize          % Make font smaller
\renewcommand{\arraystretch}{0.9}  % Reduce row spacing
\caption{Comparability Predicates (Compact Version)}
\label{tab:comparability}
\begin{tabular}{@{}M{2.4cm} M{3.2cm} P{4.0cm}@{}}
\toprule
\textbf{Predicate} & \textbf{Relation} & \textbf{Specification} \\
\midrule
\texttt{shorter}
  & subj is \textbf{shorter} than obj
  & \ length is shorter \ \texttt{delta} = height difference \\[2pt]
\texttt{longer}
  & subj is \textbf{longer} than obj
  & \ length is larger \ \texttt{delta} = length difference \\[2pt]
\texttt{taller}
  & subj is \textbf{taller} than obj
  & \ height is larger \ \texttt{delta} = height difference \\[2pt]
\texttt{thinner}
  & subj is \textbf{thinner} than obj
  & \ footprint is smaller \ \texttt{delta} = footprint difference \\[2pt]
\texttt{wider}
  & subj is \textbf{wider} than obj
  & \ footprint is larger \ \texttt{delta} = footprint difference \\[2pt]
\texttt{smaller}
  & subj is \textbf{smaller} than obj
  & \ volume is smaller \ \texttt{delta} = volume difference \\[2pt]
\texttt{bigger}
  & subj is \textbf{bigger} than obj
  & \ volume is bigger \ \texttt{delta} = volume difference \\[2pt]
\texttt{fitting}
  & subj is \textbf{fitting} into obj
  & \ is fitting within \ \texttt{delta} = volume difference \\[2pt]
\texttt{exceeding}
  & subj is \textbf{exceeding} obj
  & \ not fitting within \ \texttt{delta} = volume difference \\
\bottomrule
\end{tabular}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 10) Similarity Table
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[htbp]
\centering
\footnotesize  % Make font smaller
\renewcommand{\arraystretch}{0.9} % Reduce row spacing
\caption{Similarity Predicates (Compact Version)}
\label{tab:similarity}
\begin{tabular}{@{}M{2.4cm}M{3.8cm}P{4.0cm}@{}}
\toprule
\textbf{Predicate} & \textbf{Relation} & \textbf{Specification} \\
\midrule
\texttt{sameheight}   & subj has \textbf{sameheight} as obj   & \ height difference \(<\) max gap \\[2pt]
\texttt{samewidth}    & subj has \textbf{samewidth} as obj    & \ width difference \(<\) max gap \\[2pt]
\texttt{samedepth}    & subj has \textbf{samedepth} as obj    & \ depth difference \(<\) max gap \\[2pt]
\texttt{samelength}   & subj has \textbf{samelength} as obj   & \ length difference \(<\) max gap \\[2pt]
\texttt{sameperimeter}& subj has \textbf{sameperimeter} as obj& \ perimeter diff \(< 4\times\)(max gap) \\[2pt]
\texttt{samefront}    & subj has \textbf{samefront} as obj    & \ front area diff \(<\) (max gap)\(^2\) \\[2pt]
\texttt{sameside}     & subj has \textbf{sameside} as obj     & \ side area diff \(<\) (max gap)\(^2\) \\[2pt]
\texttt{samefootprint}& subj has \textbf{samefootprint} as obj& \ base area diff \(<\) (max gap)\(^2\) \\[2pt]
\texttt{samesurface}  & subj has \textbf{samesurface} as obj  & \ surface diff \(< 3\times\)(max gap)\(^2\) \\[2pt]
\texttt{samevolume}   & subj has \textbf{samevolume} as obj   & \ volume diff \(<\) (max gap)\(^3\) \\[2pt]
\texttt{samecuboid}   & subj has \textbf{samecuboid} as obj   & \ same width, height and depth \\[2pt]
\texttt{congruent}    & subj is \textbf{congruent} with obj   & \ same dimensions + orientation \\[2pt]
\texttt{sameposition} & subj has \textbf{sameposition} as obj & \ position diff \(<\) max gap \\[2pt]
\texttt{samecenter}   & subj has \textbf{samecenter} as obj   & \ center diff \(<\) max gap \\[2pt]
\texttt{sameshape}    & subj has \textbf{sameshape} as obj    & \ same shape label \\
\bottomrule
\end{tabular}
\end{table*}


\begin{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 11) Geography Table
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
\centering
\footnotesize          % Make font smaller
\renewcommand{\arraystretch}{0.5} 
\caption{Geography Predicates}
\label{tab:geography}
\begin{tabular}{M{2.5cm} M{3.5cm} P{4cm}}
\toprule
\textbf{Predicate} & \textbf{Relation} & \textbf{Specification} \\
\midrule
\texttt{north} 
& subj is \textbf{north} of obj
& \begin{itemize}\item center is in north direction $\pm22.5^\circ$\item valid in WCS\end{itemize} \\
%
\texttt{northeast}, \texttt{east}, \texttt{southeast}, \texttt{south}, \texttt{southwest}, \texttt{west}, \texttt{northwest}
& \textbf{dito}
& \begin{itemize}\item same principle with direction angles\end{itemize} \\
\bottomrule
\end{tabular}%
\end{table}
\end{comment}

